Enhancing Short-Text Topic Modeling with LLM-Driven Context Expansion and Prefix-Tuned VAEs

Topic modeling is a powerful technique for uncovering hidden themes within a collection of documents. However, the effectiveness of traditional topic models often relies on sufficient word co-occurrence, which is lacking in short texts. Therefore, existing approaches, whether probabilistic or neural, frequently struggle to extract meaningful patterns from such data, resulting in incoherent topics. To address this challenge, we propose a novel approach that leverages large language models (LLMs) to extend short texts into more detailed sequences before applying topic modeling. To further improve the efficiency and solve the problem of semantic inconsistency from LLM-generated texts, we propose to use prefix tuning to train a smaller language model coupled with a variational autoencoder for short-text topic modeling. Our method significantly improves short-text topic modeling performance, as demonstrated by extensive experiments on real-world datasets with extreme data sparsity, outperforming current state-of-the-art topic models.

==> tables/ClassifcationResult.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[!ht]
\resizebox{1.0\linewidth}{!}{%
\begin{tabular}{@{}ccccc|cccc|cccc|cccc|cccc@{}}
\toprule
                    & \multicolumn{4}{c}{LDA}                                                                                       & \multicolumn{4}{c}{CLNTM}                                                                                     & \multicolumn{4}{c}{CTM}                                                                                       & \multicolumn{4}{c}{NQTM}                                                                                      & \multicolumn{4}{c}{LCSNTM}                                                                                                                  \\ \midrule
                    &{MNB}   &{SVM}   &{LR}    &{RF}    &{MNB}   &{SVM}   &{LR}    &{RF}    &{MNB}   &{SVM}   &{LR}    &{RF}    & MNB                       & SVM                       & LR                        & RF                        & MNB                                & SVM                                & LR                        & RF                                 \\
                    \midrule
\multicolumn{21}{c}{StackOverflow}                                                                                                                                                                                                                                                                                                                                                                                                                                                              \\ \midrule
Short Text          &{0.643} &{0.617} &{0.643} &{0.586} &{0.051} &{0.051} &{0.066} &{0.095} &{0.807} &{\textbf{0.832}} &{0.833} &{0.770} & 0.050                     & 0.050                     & 0.050                     & 0.050                     & -                                  & -                                  & -                         & -                                  \\

Extended Text(BART) &{0.561} &{0.567} &{0.598} &{0.546} &{0.603} &{0.546} &{0.668} &{0.541} &{0.613} &{0.680} &{0.680} &{0.648} & -                         & -                         & -                         & -                         & 0.812                              & 0.824                              & 0.833                     & \textbf{0.775}                     \\

Extended Text(T5)   &{0.605} &{0.584} &{0.618} &{0.556} &{0.594} &{0.517} &{0.656} &{0.501} &{0.658} &{0.693} &{0.710} &{0.637} & -                         & -                         & -                         & -                         & \textbf{0.815}                     & 0.829                     & \textbf{0.834}            & 0.739                              \\

Extended Text(GPT-2) &{0.557} &{0.548} &{0.583} &{0.515} &{0.561} &{0.522} &{0.604} &{0.486} &{0.572} &{0.587} &{0.613} &{0.544} & -                         & -                         & -                         & -                         & 0.795                              & 0.796                              & 0.803                     & 0.695                              \\

 \midrule
\multicolumn{21}{c}{TagMyNews}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                 \\ \midrule
Short Text          & 0.335                     & 0.328                     & 0.370                     & 0.311                     & 0.254                     & 0.187                     & 0.264                     & 0.262                     & 0.564                     & 0.662                     & 0.675                     & 0.529                     & {0.274} & {0.143} & {0.278} & {0.282} & -                                  & -                                  & -                         & -                                  \\

Extended Text(BART) & 0.548                     & 0.588                     & 0.611                     & 0.491                     & 0.600                     & 0.628                     & 0.633                     & 0.470                     & 0.540                     & 0.664                     & 0.674                     & 0.524                     & -                         & -                         & -                         & -                         & {0.570}          & {0.672}          & {0.682} & {0.531}          \\

Extended Text(T5)   & 0.564                     & 0.599                     & 0.631                     & 0.477                     & \textbf{0.660}            & 0.662                     & 0.676                     & 0.509                     & 0.614                     & \textbf{0.717}            & \textbf{0.732}            & 0.557                     & -                         & -                         & -                         & -                         & {0.565}          & {0.671}          & {0.676} & {\textbf{0.557}} \\
 

Extended Text(GPT-2) & 0.550                     & 0.604                     & 0.617                     & 0.470                     & 0.611                     & 0.606                     & 0.624                     & 0.470                     & 0.505                     & 0.634                     & 0.6386                    & 0.489                     & -                         & -                         & -                         & -                         & {0.565}          & {0.650}          & {0.657} & {0.501}          \\

\midrule
\multicolumn{21}{c}{WebSnippets}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                               \\ \midrule
Short Text          & 0.531                     & 0.575                     & 0.591                     & 0.402                     & 0.215                     & 0.150                     & 0.472                     & \textbf{0.716}                     & 0.712                     & 0.850                     & \textbf{0.856}            & 0.632                     & {0.397} & {0.380} & {0.438} & {0.376} & -                                  & -                                  & -                         & -                                  \\

Extended Text(BART) & 0.547                     & 0.621                     & 0.628                     & 0.486                     & 0.653                     & 0.765                     & 0.773                     & 0.603                     & 0.589                     & 0.792                     & 0.799                     & 0.628                     & -                         & -                         & -                         & -                         & {\textbf{0.720}} & {0.829}          & {0.850} & {0.678} \\

Extended Text(T5)   & 0.657                     & 0.717                     & 0.724                     & 0.532                     & 0.712                     & 0.801                     & 0.820                     & 0.648                     & 0.696                     & 0.826                     & 0.843                     & 0.601                     & -                         & -                         & -                         & -                         & {0.703}          & {\textbf{0.852}} & {0.852} & {0.647}          \\

Extended Text(GPT-2) & 0.564                     & 0.637                     & 0.640                     & 0.532                     & 0.529                     & 0.695                     & 0.696                     & 0.607                     & 0.495                     & 0.701                     & 0.690                     & 0.546                     & -                         & -                         & -                         & -                         & {0.654}          & {0.817}          & {0.820} & {0.682}          \\

 \bottomrule
\end{tabular}}
\caption{Text classification accuracy over 5-fold cross validation. The best results in each case are shown in \textbf{bold}.}
\label{tab:classification}
\vspace{-1mm}
\end{table*}

==> tables/TQ_detail.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[!ht]
\centering
\resizebox{1.0\linewidth}{!}{%
\begin{tabular}{@{}cccc|cc|cc|cc|cc|cc|cc@{}}
\toprule
\multirow{3}{*}{Data}                & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Topic\\ Quality\\ Metrics\end{tabular}} & \multicolumn{6}{c}{General Purpose Topic Models}                              & \multicolumn{6}{c}{Short Text Topic Models}                                                                                  & \multicolumn{2}{c}{\multirow{3}{*}{LCSNTM}} \\ \cmidrule(lr){3-14}
                                     &                                                                                    & \multicolumn{2}{c}{LDA} & \multicolumn{2}{c}{CLNTM} & \multicolumn{2}{c}{CTM} & \multicolumn{2}{c}{BTM} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Graph\\ BTM\end{tabular}} & \multicolumn{2}{c}{NQTM} & \multicolumn{2}{c}{}                      \\ \cmidrule(l){3-16} 
                                     &                                                                                    & k=20        & k=50      & k=20        & k=50        & k=20       & k=50       & k=20       & k=50       & k=20                               & k=50                               & k=20       & k=50        & k=20                & k=50                \\ \midrule
\multicolumn{16}{c}{StackOverflow}                                                                                                                                                                                                                                                                                                                                                                        \\ \midrule
\multirow{3}{*}{Short Text}               & {NPMI}                                                           & 0.041  & 0.011          & -0.074         & -0.141         & 0.021          & 0.099          & 0.062      & 0.074      & -0.154                             & -0.183                             & -0.08       & -0.099     & -                    & -                    \\
                                          & CWE                                                                                & 0.129  & 0.120          & 0.124          & 0.111          & 0.139          & 0.135          & 0.137      & 0.138      & 0.096                              & 0.097                              & 0.119       & 0.099      & -                    & -                    \\
                                          & IRBO                                                                                & 0.985  & 0.989          & 0.814          & 0.925          & 0.995          & 0.979          & 0.889      & 0.920      & 0.790                              & 0.952                              & 0.990       & 0.992      & -                    & -                    \\ \midrule
\multirow{3}{*}{Extended Text(BART)}      & {NPMI}                                                           & 0.042  & 0.014          & -0.054         & -0.051         & 0.034          & 0.056          & -          & -          & -                                  & -                                  & -           & -          & \textbf{0.101}       & \textbf{0.109}       \\ 
                                          & CWE                                                                                & 0.138  & 0.131          & 0.140          & 0.150          & \textbf{0.153}          & \textbf{0.155}          & -          & -          & -                                  & -                                  & -           & -          & 0.139                & 0.139                \\
                                          & IRBO                                                                                & 0.998  & \textbf{0.998} & \textbf{1.0}   & 0.996 & \textbf{1.0}   & 0.994          & -          & -          & -                                  & -                                  & -           & -          & 0.995                & 0.979                \\  \cmidrule(l){2-16}
\multirow{3}{*}{Extended Text(T5)}        & {NPMI}                                                           & 0.066  & 0.054          & 0.017          & 0.029          & 0.101          & \textbf{0.109} & -          & -          & -                                  & -                                  & -           & -          & \textbf{0.109}       & \textbf{0.109}       \\
                                          & CWE                                                                                & 0.139  & 0.145          & \textbf{0.174} & \textbf{0.167} & 0.139          & 0.157 & -          & -          & -                                  & -                                  & -           & -          & 0.137                & 0.140       \\
                                          & IRBO                                                                                & 0.998  & \textbf{0.997} & 0.997          & 0.996          & \textbf{1.0}   & 0.994          & -          & -          & -                                  & -                                  & -           & -          & 0.995                & 0.976                \\ \cmidrule(l){2-16}
\multirow{3}{*}{Extended Text(GPT-2)}      & {NPMI}                                                           & 0.08   & 0.089          & 0.005          & -0.007         & 0.094          & 0.098          & -          & -          & -                                  & -                                  & -           & -          & \textbf{0.102}       & \textbf{0.115}       \\
                                          & CWE                                                                                & 0.158  & 0.153          & \textbf{0.172}          & \textbf{0.178} & 0.148          & 0.158          & -          & -          & -                                  & -                                  & -           & -          & 0.145                & 0.140      \\
                                          & IRBO                                                                                & 0.990  & 0.992          & \textbf{0.999} & 0.996          & \textbf{0.996} & 0.995          & -          & -          & -                                  & -                                  & -           & -          & 0.988                & 0.967                \\ \midrule
\multicolumn{16}{c}{TagMyNews}                                                                                                                                                                                                                                                                                                                                                                            \\ \midrule
\multirow{3}{*}{Short Text}               & {NPMI}                                                           & -0.040 & -0.062         & -0.063         & -0.086         & -0.009         & -0.006         & -0.032     & -0.029     & -0.134                             & -0.140                             & -0.059      & -0.057     & -                    & -                    \\
                                          & CWE                                                                                & 0.107  & 0.096          & 0.104          & 0.088          & 0.158          & 0.164          & 0.127      & 0.124      & 0.072                              & 0.074                              & 0.095       & 0.092      & -                    & -                    \\
                                          & IRBO                                                                                & 0.998  & 0.999          & 0.752          & 0.978          & 0.996          & 0.982          & 0.971      & 0.975      & 0.960                              & 0.986                              & 0.959       & 0.951      & -                    & -                    \\ \midrule
\multirow{3}{*}{Extended Text(BART)}      & {NPMI}                                                           & 0.019  & 0.016          & 0.014          & 0.033          & \textbf{0.046} & \textbf{0.040} & -          & -          & -                                  & -                                  & -           & -          & 0.015                & 0.007                \\
                                          & CWE                                                                                & 0.171  & 0.163          & \textbf{0.247} & \textbf{0.208} & 0.199          & 0.197          & -          & -          & -                                  & -                                  & -           & -          & 0.168                & 0.165       \\
                                          & IRBO                                                                                & 0.983  & 0.993          & \textbf{1.000} & 0.996          & 0.999 & \textbf{0.995} & -          & -          & -                                  & -                                  & -           & -          & 0.992                & 0.983                \\
                                           \cmidrule(l){2-16}
\multirow{3}{*}{Extended Text(T5)}        & {NPMI}                                                           & -0.001 & -0.012         & -0.022         & 0.016          & \textbf{0.034} & \textbf{0.039} & -          & -          & -                                  & -                                  & -           & -          & 0.007                & 0.012                \\
                                          & CWE                                                                                & 0.156  & 0.153          & \textbf{0.252} & \textbf{0.215} & 0.211          & 0.201          & -          & -          & -                                  & -                                  & -           & -          & 0.161                & 0.153       \\
                                          & IRBO                                                                                & 0.964  & 0.990          & \textbf{1.000} & \textbf{0.997} & 0.999          & 0.994          & -          & -          & -                                  & -                                  & -           & -          & 0.993                & 0.978                \\ \cmidrule(l){2-16}
\multirow{3}{*}{Extended Text(GPT-2)}      & {NPMI}                                                           & 0.035  & 0.031          & 0.018          & \textbf{0.066} & \textbf{0.065} & 0.054          & -          & -          & -                                  & -                                  & -           & -          & 0.009                & 0.001                \\
                                          & CWE                                                                                & 0.198  & 0.185          & \textbf{0.273} & \textbf{0.253}          & 0.231          & 0.222          & -          & -          & -                                  & -                                  & -           & -          & 0.162                & 0.162                \\
                                          & IRBO                                                                                & 0.951  & 0.981          & \textbf{1.000} & \textbf{0.998} & 0.999          & 0.994          & -          & -          & -                                  & -                                  & -           & -          & 0.985                & 0.971                \\ \midrule
\multicolumn{16}{c}{WebSnippets}                                                                                                                                                                                                                                                                                                                                                                          \\ \midrule
\multirow{3}{*}{Short Text}               & {NPMI}                                                           & -0.045 & -0.061         & -0.110         & -0.059         & 0.002          & 0.001          & 0.009      & 0.01       & -0.154                             & -0.136                             & -0.177      & -0.156     & -                    & -                    \\
                                          & CWE                                                                                & 0.163  & 0.144          & 0.248          & 0.188          & 0.209          & 0.224          & 0.192      & 0.188      & 0.115                              & 0.107                              & 0.096       & 0.091      & -                    & -                    \\
                                          & IRBO                                                                                & 0.995  & 0.997          & \textbf{1.000}          & 0.759          & 0.999          & 0.998          & 0.918      & 0.953      & 0.944                              & 0.972                              & 0.996       & 0.992      & -                    & -                    \\ \midrule
\multirow{3}{*}{Extended Text(BART)}      & {NPMI}                                                           & -0.019 & -0.039         & -0.092         & -0.090         & \textbf{0.030} & 0.001          & -          & -          & -                                  & -                                  & -           & -          & 0.025                & \textbf{0.109}       \\
                                          & CWE                                                                                & 0.150  & 0.155          & 0.202          & 0.208          & 0.219          & 0.210          & -          & -          & -                                  & -                                  & -           & -          & \textbf{0.226}       & 0.220                \\
                                          & IRBO                                                                                & 0.996  & \textbf{0.999} & 0.999          & 0.998          & \textbf{1.000}          & 0.997          & -          & -          & -                                  & -                                  & -           & -          & \textbf{1.000}       & 0.996                \\ \cmidrule(l){2-16}
\multirow{3}{*}{Extended Text(T5)}        & {NPMI}                                                           & 0.008  & -0.035         & -0.095         & -0.074         & \textbf{0.033} & 0.013          & -          & -          & -                                  & -                                  & -           & -          & 0.012                & \textbf{0.115}       \\
                                          & CWE                                                                                & 0.193  & 0.170          & 0.230          & 0.230          & \textbf{0.246} & 0.234          & -          & -          & -                                  & -                                  & -           & -          & 0.234                & 0.221                \\
                                          & IRBO                                                                                & 0.996  & 0.998          & 0.999 & 0.998          & \textbf{1.000} & \textbf{1.000} & -          & -          & -                                  & -                                  & -           & -          & \textbf{1.000}       & 0.995                \\ \cmidrule(l){2-16}
\multirow{3}{*}{Extended Text(GPT-2)}      & {NPMI}                                                           & 0.013  & -0.024         & -0.048         & -0.058         & 0.020          & 0.008          & -          & -          & -                                  & -                                  & -           & -          & \textbf{0.028}       & \textbf{0.109}       \\
                                          & CWE                                                                                & 0.202  & 0.181          & 0.232          & \textbf{0.246} & \textbf{0.250} & 0.234          & -          & -          & -                                  & -                                  & -           & -          & 0.241                & 0.221                \\
                                          & IRBO                                                                                & 0.998  & \textbf{0.999} & 0.999          & 0.998          & \textbf{1.000} & 0.996          & -          & -          & -                                  & -                                  & -           & -          & \textbf{1.000}       & 0.993                \\  \bottomrule 
\end{tabular}
}
\caption{Topic coherences (NPMI and CWE) and diversity (IRBO) scores of topic words. $k$ is the topic number. The best in each case is shown in \textbf{bold}.}
\label{tab:topic_quality}
% \vspace{-1mm}
\end{table*}

==> tables/TQresult.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[!ht]
\centering
\resizebox{1.0\linewidth}{!}{%
\begin{tabular}{@{}c|c|cc|cc|cc|cc|cc|cc|cc@{}}
\toprule
\multirow{3}{*}{Data}                & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Topic\\ Quality\\ Metrics\end{tabular}} & \multicolumn{6}{c}{General Purpose Topic Models}                              & \multicolumn{6}{c}{Short Text Topic Models}                                                                                  & \multicolumn{2}{c}{\multirow{2}{*}{LCSNTM}} \\ \cmidrule(lr){3-14}
                                     &                                                                                    & \multicolumn{2}{c}{LDA} & \multicolumn{2}{c}{CLNTM} & \multicolumn{2}{c}{CTM} & \multicolumn{2}{c}{BTM} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Graph\\ BTM\end{tabular}} & \multicolumn{2}{c}{NQTM} & \multicolumn{2}{c}{}                      \\ \cmidrule(l){3-16} 
                                     &                                                                                    & k=20        & k=50      & k=20        & k=50        & k=20       & k=50       & k=20       & k=50       & k=20                               & k=50                               & k=20       & k=50        & k=20                & k=50                \\ \midrule
\multicolumn{16}{c}{StackOverflow}                                                                                                                                                                                                                                                                                                                                                                   \\ \midrule
\multirow{2}{*}{Short Text}          & NPMI                                                                               & 0.041  & 0.011          & -0.074         & -0.141         & 0.101          & 0.099          & 0.062      & 0.074      & -0.154                             & -0.183                             & -0.08       & -0.099     & -                    & -                    \\
                                     & RBO                                                                                & 0.985  & 0.989          & 0.814          & 0.925          & 0.995          & 0.979          & 0.927      & 0.92       & 0.790                              & 0.952                              & 0.99        & 0.992      & -                    & -                    \\ \midrule
\multirow{2}{*}{Extended Text (GPT2)} & NPMI                                                                               & 0.08   & 0.089          & 0.005          & -0.007         & 0.094          & 0.098          & -          & -          & -                                  & -                                  & -           & -          & \textbf{0.102}       & \textbf{0.115}       \\
                                     & RBO                                                                                & 0.99   & 0.992          & \textbf{0.998} & \textbf{0.996} & 0.996          & 0.994          & -          & -          & -                                  & -                                  & -           & -          & 0.988                & 0.967                \\ \cmidrule(l){2-16} 
\multirow{2}{*}{Extended Text (T5)}   & NPMI                                                                               & 0.066  & 0.054          & 0.017          & 0.029          & 0.101          & \textbf{0.109} & -          & -          & -                                  & -                                  & -           & -          & \textbf{0.109}       & \textbf{0.109}       \\
                                     & RBO                                                                                & 0.998  & \textbf{0.997} & 0.997          & 0.996          & \textbf{0.999} & 0.994          & -          & -          & -                                  & -                                  & -           & -          & 0.995                & 0.976                \\ \cmidrule(l){2-16} 
\multirow{2}{*}{Extended Text(BART)} & NPMI                                                                               & 0.042  & 0.014          & -0.054         & -0.051         & 0.034          & 0.056          & -          & -          & -                                  & -                                  & -           & -          & \textbf{0.101}       & \textbf{0.109}       \\
                                     & RBO                                                                                & 0.998  & \textbf{0.998} & 0.999          &                & \textbf{0.999} & 0.994          & -          & -          & -                                  & -                                  & -           & -          & 0.995                & 0.978                \\ \midrule
\multicolumn{16}{c}{TagMyNews}                                                                                                                                                                                                                                                                                                                                                                       \\ \midrule
\multirow{2}{*}{Short Text}          & NPMI                                                                               & -0.040 & -0.062         & -0.063         & -0.086         & -0.009         & -0.006         & -0.032     & -0.029     & -0.134                             & -0.140                             & -0.059      & -0.057     & -                    & -                    \\
                                     & RBO                                                                                & 0.997  & 0.915          & 0.752          & 0.978          & 0.996          & 0.982          & 0.971      & 0.975      & 0.960                              & 0.986                              & 0.959       & 0.951      & -                    & -                    \\ \midrule
\multirow{2}{*}{Extended Text(GPT2)} & NPMI                                                                               & 0.035  & 0.031          & 0.018          & \textbf{0.066} & \textbf{0.065} & 0.054          & -          & -          & -                                  & -                                  & -           & -          & 0.009                & 0.001                \\
                                     & RBO                                                                                & 0.951  & 0.981          & 0.999          & 0.998          & \textbf{0.999} & \textbf{0.994} & -          & -          & -                                  & -                                  & -           & -          & 0.985                & 0.971                \\
\multirow{2}{*}{Extended Text(T5)}   & NPMI                                                                               & -0.001 & -0.012         & -0.022         & 0.016          & \textbf{0.034} & \textbf{0.039} & -          & -          & -                                  & -                                  & -           & -          & 0.007                & 0.012                \\
                                     & RBO                                                                                & 0.964  & 0.990          & \textbf{1.0}   & \textbf{0.997} & 0.999          & 0.994          & -          & -          & -                                  & -                                  & -           & -          & 0.993                & 0.978                \\
\multirow{2}{*}{Extended Text(BART)} & NPMI                                                                               & 0.019  & 0.016          & 0.014          & 0.033          & \textbf{0.046} & \textbf{0.040} & -          & -          & -                                  & -                                  & -           & -          & 0.015                & 0.007                \\
                                     & RBO                                                                                & 0.983  & 0.993          & \textbf{1.0}   & \textbf{0.996} & 0.999          & 0.995          & -          & -          & -                                  & -                                  & -           & -          & 0.992                & 0.983                \\ \midrule
\multicolumn{16}{c}{WebSnippets}                                                                                                                                                                                                                                                                                                                                                                     \\ \midrule
\multirow{2}{*}{Short Text}          & NPMI                                                                               & -0.045 & -0.061         & -0.110         & -0.059         & 0.002          & 0.001          & 0.009      & 0.01       & -0.154                             & -0.136                             & -0.177      & -0.156     & -                    & -                    \\
                                     & RBO                                                                                & 0.994  & 0.997          & 0.999          & 0.759          & 0.999          & 0.998          & 0.918      & 0.953      & 0.944                              & 0.972                              & 0.996       & 0.992      & -                    & -                    \\ \midrule
\multirow{2}{*}{Extended Text(GPT2)} & NPMI                                                                               & 0.013  & -0.024         & -0.048         & -0.058         & 0.020          & 0.008          & -          & -          & -                                  & -                                  & -           & -          & \textbf{0.028}       & \textbf{0.109}       \\
                                     & RBO                                                                                & 0.998  & \textbf{0.999} & 0.999          & 0.997          & 0.999          & 0.996          & -          & -          & -                                  & -                                  & -           & -          & \textbf{1.0}         & 0.978                \\ \cmidrule(l){2-16} 
\multirow{2}{*}{Extended Text(T5)}   & NPMI                                                                               & 0.008  & -0.035         & -0.095         & -0.074         & \textbf{0.033} & 0.013          & -          & -          & -                                  & -                                  & -           & -          & 0.012                & \textbf{0.115}       \\
                                     & RBO                                                                                & 0.996  & 0.998          & \textbf{0.999} & 0.998          & \textbf{1.0}   & \textbf{0.999} & -          & -          & -                                  & -                                  & -           & -          & \textbf{1.0}         & 0.967                \\ \cmidrule(l){2-16} 
\multirow{2}{*}{Extended Text(BART)} & NPMI                                                                               & -0.019 & -0.039         & -0.092         & -0.090         & \textbf{0.030} & 0.001          & -          & -          & -                                  & -                                  & -           & -          & 0.025                & \textbf{0.109}       \\
                                     & RBO                                                                                & 0.995  & 0.999          & \textbf{0.999} & 0.998          & \textbf{1.0}   & 0.997          & -          & -          & -                                  & -                                  & -           & -          & \textbf{1.0}         & 0.977                \\  \bottomrule 
\end{tabular}
}
\caption{Topic coherence (NPMI) and diversity (RBO) scores of topic words. $k$ is the topic number. The best in each case is shown in \textbf{bold}.}
\label{tab:topic_quality}
\end{table*}

==> tables/TQstackoverflow.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[]
\centering
\resizebox{1.0\linewidth}{!}{%
\begin{tabular}{@{}c|c|cc|cc|cc|cc|cc|cc|cc@{}}
\toprule
\multirow{3}{*}{Data}                & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Topic\\ Quality\\ Metrics\end{tabular}} & \multicolumn{6}{c}{General Purpose Topic Models}                              & \multicolumn{6}{c}{Short Text Topic Models}                                                                                  & \multicolumn{2}{c}{\multirow{2}{*}{Ours}} \\ \cmidrule(lr){3-14}
                                     &                                                                                    & \multicolumn{2}{c}{LDA} & \multicolumn{2}{c}{CLNTM} & \multicolumn{2}{c}{CTM} & \multicolumn{2}{c}{BTM} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Graph\\ BTM\end{tabular}} & \multicolumn{2}{c}{NQTM} & \multicolumn{2}{c}{}                      \\ \cmidrule(l){3-16} 
                                     &                                                                                    & k=20        & k=50      & k=20        & k=50        & k=20       & k=50       & k=20       & k=50       & k=20                               & k=50                               & k=20       & k=50        & k=20                & k=50                \\ \midrule
\multirow{2}{*}{Short Text}          & NPMI                                                                               & 0.041       & 0.011     & -0.074      & -0.141      & 0.101      & 0.099      & 0.062      & 0.074      &                                    &                                    & -0.08      & -0.099      &                     &                     \\
                                     & RBO                                                                                & 0.985       & 0.989     & 0.814       & 0.925       & 0.995      & 0.979      & 0.927      & 0.92       &                                    &                                    & 0.99       & 0.992       &                     &                     \\
\multirow{2}{*}{Extended Text(GPT2)} & NPMI                                                                               & 0.08        & 0.089     & 0.005       & -0.007      & 0.094      & 0.098      &            &            &                                    &                                    &            &             & 0.102               & 0.115               \\
                                     & RBO                                                                                & 0.99        & 0.992     & 0.998       & 0.996       & 0.996      & 0.994      &            &            &                                    &                                    &            &             & 0.988               & 0.967               \\
\multirow{2}{*}{Extended Text(T5)}   & NPMI                                                                               & 0.066       & 0.054     & 0.017       & 0.029       & 0.101      & 0.109      &            &            &                                    &                                    &            &             & 0.109               & 0.109               \\
                                     & RBO                                                                                & 0.998       & 0.997     & 0.997       & 0.996       & 0.999      & 0.994      &            &            &                                    &                                    &            &             & 0.995               & 0.976               \\
\multirow{2}{*}{Extended Text(BART)} & NPMI                                                                               & 0.042       & 0.014     & -0.054      & -0.051      & 0.034      & 0.056      &            &            &                                    &                                    &            &             & 0.101               & 0.109               \\
                                     & RBO                                                                                & 0.998       & 0.998     & 0.999       & 0.996       & 0.999      & 0.994      &            &            &                                    &                                    &            &             & 0.995               & 0.978               \\ \bottomrule 
\end{tabular}
}
\end{table*}

==> tables/TQtagmynews.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[]
\centering
\resizebox{1.0\linewidth}{!}{%
\begin{tabular}{@{}c|c|cc|cc|cc|cc|cc|cc|cc@{}}
\toprule
\multirow{3}{*}{Data}                & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Topic\\ Quality\\ Metrics\end{tabular}} & \multicolumn{6}{c}{General Purpose Topic Models}                              & \multicolumn{6}{c}{Short Text Topic Models}                                                                                  & \multicolumn{2}{c}{\multirow{2}{*}{Ours}} \\ \cmidrule(lr){3-14}
                                     &                                                                                    & \multicolumn{2}{c}{LDA} & \multicolumn{2}{c}{CLNTM} & \multicolumn{2}{c}{CTM} & \multicolumn{2}{c}{BTM} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Graph\\ BTM\end{tabular}} & \multicolumn{2}{c}{NQTM} & \multicolumn{2}{c}{}                      \\ \cmidrule(l){3-16} 
                                     &                                                                                    & k=20        & k=50      & k=20        & k=50        & k=20       & k=50       & k=20       & k=50       & k=20                               & k=50                               & k=20       & k=50        & k=20                & k=50                \\ \midrule
\multirow{2}{*}{Short Text}          & NPMI                                                                               & -0.040     & -0.062     & -0.063      & -0.086      & -0.009     & -0.006     & -0.032     & -0.029     &                                    &                                    & -0.059      & -0.057     &                      &                    \\
                                     & RBO                                                                                & 0.997      & 0.915      & 0.752       & 0.978       & 0.996      & 0.982      & 0.971      & 0.975      &                                    &                                    & 0.959       & 0.951      &                      &                    \\
\multirow{2}{*}{Extended Text(GPT2)} & NPMI                                                                               & 0.035      & 0.031      & 0.018       & 0.066       & 0.065      & 0.054      &            &            &                                    &                                    &             &            & -0.009               & 0.115              \\
                                     & RBO                                                                                & 0.951      & 0.981      & 0.999       & 0.998       & 0.999      & 0.994      &            &            &                                    &                                    &             &            & 0.985                & 0.967              \\
\multirow{2}{*}{Extended Text(T5)}   & NPMI                                                                               & -0.001     & -0.012     & -0.022      & 0.016       & 0.034      & 0.039      &            &            &                                    &                                    &             &            & -0.006               & 0.108              \\
                                     & RBO                                                                                & 0.964      & 0.990      & 1.0         & 0.997       & 0.999      & 0.994      &            &            &                                    &                                    &             &            & 0.993                & 0.976              \\
\multirow{2}{*}{Extended Text(BART)} & NPMI                                                                               & 0.019      & 0.016      & 0.014       & 0.033       & 0.046      & 0.040      &            &            &                                    &                                    &             &            & -0.193               & 0.109              \\
                                     & RBO                                                                                & 0.983      & 0.993      & 1.0         & 0.996       & 0.999      & 0.995      &            &            &                                    &                                    &             &            & 0.992                & 0.977              \\ \bottomrule 
\end{tabular}
}
\end{table*}

==> tables/TQwebsnippets.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[]
\centering
\resizebox{1.0\linewidth}{!}{%
\begin{tabular}{@{}c|c|cc|cc|cc|cc|cc|cc|cc@{}}
\toprule
\multirow{3}{*}{Data}                & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Topic\\ Quality\\ Metrics\end{tabular}} & \multicolumn{6}{c}{General Purpose Topic Models}                              & \multicolumn{6}{c}{Short Text Topic Models}                                                                                  & \multicolumn{2}{c}{\multirow{2}{*}{Ours}} \\ \cmidrule(lr){3-14}
                                     &                                                                                    & \multicolumn{2}{c}{LDA} & \multicolumn{2}{c}{CLNTM} & \multicolumn{2}{c}{CTM} & \multicolumn{2}{c}{BTM} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Graph\\ BTM\end{tabular}} & \multicolumn{2}{c}{NQTM} & \multicolumn{2}{c}{}                      \\ \cmidrule(l){3-16} 
                                     &                                                                                    & k=20        & k=50      & k=20        & k=50        & k=20       & k=50       & k=20       & k=50       & k=20                               & k=50                               & k=20       & k=50        & k=20                & k=50                \\ \midrule
\multirow{2}{*}{Short Text}          & NPMI                                                                               & -0.045     & -0.061     & -0.110      & -0.059      & 0.002      & 0.001      & 0.009      & 0.01       &                                    &                                    & -0.177      & -0.156     &                     &                     \\
                                     & RBO                                                                                & 0.994      & 0.997      & 0.999       & 0.759       & 0.999      & 0.998      & 0.918      & 0.953      &                                    &                                    & 0.996       & 0.992      &                     &                     \\
\multirow{2}{*}{Extended Text(GPT2)} & NPMI                                                                               & 0.013      & -0.024     & -0.048      & -0.058      & 0.020      & 0.008      &            &            &                                    &                                    &             &            & 0.028               & 0.109               \\
                                     & RBO                                                                                & 0.998      & 0.999      & 0.999       & 0.997       & 0.999      & 0.996      &            &            &                                    &                                    &             &            & 1.0                 & 0.978               \\
\multirow{2}{*}{Extended Text(T5)}   & NPMI                                                                               & 0.008      & -0.035     & -0.095      & -0.074      & 0.033      & 0.013      &            &            &                                    &                                    &             &            & 0.012               & 0.115               \\
                                     & RBO                                                                                & 0.996      & 0.998      & 0.999       & 0.998       & 1.0        & 0.999      &            &            &                                    &                                    &             &            & 1.0                 & 0.967               \\
\multirow{2}{*}{Extended Text(BART)} & NPMI                                                                               & -0.019     & -0.039     & -0.092      & -0.090      & 0.030      & 0.001      &            &            &                                    &                                    &             &            & 0.025               & 0.109               \\
                                     & RBO                                                                                & 0.995      & 0.999      & 0.999       & 0.998       & 1.0        & 0.997      &            &            &                                    &                                    &             &            & 0.999               & 0.977               \\ \bottomrule 
\end{tabular}
}
\end{table*}

==> tables/errorexample.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \begin{table*}[]
% \resizebox{1.0\linewidth}{!}{%
% \begin{tabular}{@{}ll@{}}
% \toprule
% Short Text                  & court agrees to expedite n.f.l.'s appeal                                                                                                \\ \midrule
% Generated Long Text (GPT2) & \begin{tabular}[c]{@{}l@{}}court agrees to expedite N.F.L. appeal.May 5, 1987 The Third United States Circuit Court of Appeals issues an \\order denying Enron's request for summary judgment in his suit seeking summary judgment from Enron in his\\ suit for injunctive relief to prevent Enron from misusing the trademark ""energy"" in commerce. Judge Joseph S.\\ Tumlinson's order states that both plaintiffs are estopped from arguing, pursuant to Fed.R.Civ.P....\end{tabular} \\ \bottomrule
% \end{tabular}}
% \caption{Example extended text generated using GPT2 from TagMyNews dataset.}
% \label{tab:error_example}
% \end{table*}


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[!ht]
\resizebox{1.0\linewidth}{!}{%
\begin{tabular}{@{}lll@{}}
\toprule
\begin{tabular}[c]{@{}l@{}}Short \\ Texts\end{tabular}    & no tsunami but fifa's corruption storm rages on                                                                                                                                                                                                                                                                                                                                                                                                              & court agrees to expedite n.f.l.'s appeal                                                                                                                                                                                                                                                                                                                                                                                                     \\ \midrule
\begin{tabular}[c]{@{}l@{}}Extended \\ Texts\end{tabular} & \begin{tabular}[c]{@{}l@{}}no tsunami but fifa's corruption storm rages on. fifa president \\ sepp blatter speaks out about corruption scandals . but fifa's \\ stewardship is far from over and fifa are not at fault . Fernando \\ torres, fifa's head of integrity, is still alive and kicking . fa and \\ fifa must stop corruption before fifa takes over . fifa fans are not \\ safe when it comes to their vote, this is not the place..\end{tabular} & \begin{tabular}[c]{@{}l@{}}court agrees to expedite N.F.L. appeal.May 5, 1987. The Third \\ United States Circuit Court of Appeals issues an order denying\\ Enron's request for summary judgment in his suit seeking summary\\ judgment from Enron in his  suit for injunctive relief to prevent Enron \\ from misusing the trademark ""energy"" in commerce.\\ Judge Joseph S.Tumlinson's order states that both plaintiffs..\end{tabular} \\ \bottomrule
\end{tabular}}
\caption{Example short texts and corresponding extended texts using PLMs.}
\label{tab:error_example}
\end{table*}




==> tables/length_effect.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\resizebox{1.0\linewidth}{!}{%
\begin{tabular}{@{}l|l|l|l|l@{}}
\toprule
\multicolumn{1}{c}{Text-Length} & 20     & 30     & 50     & 100   \\ \midrule
\multicolumn{5}{c}{Stack Overflow}                                 \\ \midrule
NPMI                            & 0.072  & 0.077  & 0.082  & 0.083 \\
CWE                             & 0.157  & 0.158  & 0.159  & 0.153 \\
IRBO                            & 0.992  & 0.992  & 0.992  & 0.994 \\ \midrule
\multicolumn{5}{c}{TagMyNews}                                      \\ \midrule
NPMI                            & 0.032  & 0.037  & 0.044  & 0.045 \\
CWE                             & 0.189  & 0.201  & 0.199  & 0.201 \\
IRBO                            & 0.991  & 0.992  & 0.992  & 0.990 \\ \midrule
\multicolumn{5}{c}{WebSnippets}                                    \\ \midrule
NPMI                            & -0.015 & -0.028 & -0.008 & 0.008 \\
CWE                             & 0.227  & 0.212  & 0.237  & 0.234 \\
IRBO                            & 0.992  & 0.990  & 0.992  & 0.996 \\ \bottomrule
\end{tabular}}
\caption{Effect of generated text length on Topic quality}
\label{tab:length}
\end{table}
